Reinforced Approximate Exploratory Data Analysis

Exploratory data analytics (EDA) is a sequential decision making process where analysts choose subsequent queries that might lead to some interesting insights based on the previous queries and corresponding results. Data processing systems often execute the queries on samples to produce results with low latency. Different downsampling strategy preserves different statistics of the data and have different magnitude of latency reductions. The optimum choice of sampling strategy often depends on the particular context of the analysis flow and the hidden intent of the analyst. In this paper, we are the first to consider the impact of sampling in interactive data exploration settings as they introduce approximation errors. We propose a Deep Reinforcement Learning (DRL) based framework which can optimize the sample selection in order to keep the analysis and insight generation flow intact. Evaluations with 3 real datasets show that our technique can preserve the original insight generation flow while improving the interaction latency, compared to baseline methods.

==> sec_temp.tex <==
\section{Results}
\subsection{Experimental Setup}
\subsubsection{Flight-Delays Dataset}
We use a dataset derived from the popular flight-delays dataset. This dataset contains records of past flights with attributes such as origin airport, destination airport, delay reason, etc. This dataset was also used by \cite{atena2020sigmod} and we use their simulator to generate sequences as close to human analyst as possible. We use around $\sim 500k$ rows from this dataset to train the simulator. Then 6000 unique sequences are generated for this dataset by the simulator and we train our RL agent using two strategies. In the first, we train the RL agent on all generated sequences and in the second, we holdout a set of 1200 sequences and train our RL agent on remaining 4800 sequences.

\begin{figure*}[t]
\centering
\begin{minipage}{1.0\textwidth}
%\includegraphics[width=1.0\linewidth]{figures/intent_divergence.png}
\includegraphics[width=0.7\linewidth]{figures/junk_topic_model.png}
     \caption{Results of topic modeling on Flights data.}
     %\label{fig:top_distribution}
\end{minipage}
\begin{minipage}{1.0\textwidth}
%\includegraphics[width=1.0\linewidth]{figures/intent_divergence.png}
\includegraphics[width=1.0\linewidth]{figures/junk_motivation.png}
     \caption{Results showing how the distribution of topics change if EDA is used on sampled data.}
     %\label{fig:top_distribution}
\end{minipage}
\end{figure*}
\begin{figure*}[t]
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{figures/junk_reward_comparison.png}
\caption{Comparison of RL-reward for different distance metrics}
%\label{fig:framework}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{figures/junk_reward.png}
\caption{Characteristics of reward for RL training.}
%\label{fig:framework}
\end{minipage}
\end{figure*}


